Blocks2World: Controlling Realistic Scenes with Editable Primitives

We present Blocks2World, a novel method for 3D scene rendering and editing that leverages a two-step process: convex decomposition of images and conditioned synthesis. Our technique begins by extracting 3D parallelepipeds from various objects in a given scene using convex decomposition, thus obtaining a primitive representation of the scene. These primitives are then utilized to generate paired data through simple ray-traced depth maps. The next stage involves training a conditioned model that learns to generate images from the 2D-rendered convex primitives. This step establishes a direct mapping between the 3D model and its 2D representation, effectively learning the transition from a 3D model to an image. Once the model is fully trained, it offers remarkable control over the synthesis of novel and edited scenes. This is achieved by manipulating the primitives at test time, including translating or adding them, thereby enabling a highly customizable scene rendering process. Our method provides a fresh perspective on 3D scene rendering and editing, offering control and flexibility. It opens up new avenues for research and applications in the field, including authoring and data augmentation.

==> sections/others-daf.tex <==
\section{Limitations}
We tried training a model with semantic segmentation conditioning. 

Show a figure with ControlNet struggling to give us what we want. Refer to previous ICCV paper to get a sense of how simple the primitives are compared to the GT.

A larger primitive-image training dataset to condition the neural renderer will improve the image quality particularly for less frequent scene labels. 



\section{Conclusion}
